Algorithms with Prediction Portfolios

The research area of algorithms with predictions has seen recent success showing how to incorporate machine learning into algorithm design to improve performance when the predictions are correct, while retaining worst-case guarantees when they are not. Most previous work has assumed that the algorithm has access to a single predictor. However, in practice, there are many machine learning methods available, often with incomparable generalization guarantees, making it hard to pick a best method a priori. In this work we consider scenarios where multiple predictors are available to the algorithm and the question is how to best utilize them. Ideally, we would like the algorithm's performance to depend on the quality of the best predictor. However, utilizing more predictions comes with a cost, since we now have to identify which prediction is the best. We study the use of multiple predictors for a number of fundamental problems, including matching, load balancing, and non-clairvoyant scheduling, which have been well-studied in the single predictor setting. For each of these problems we introduce new algorithms that take advantage of multiple predictors, and prove bounds on the resulting performance.

==> prelim.tex <==
\section{Learnability}
\label{sec:prelim}
When designing new methods in the algorithms with predictions setting, the predictions under consideration must satisfy two constraints.  First, they should be useful to the algorithm, so that using the predictions allows the algorithm to achieve better running time, competitive ratio, or some other performance measure. Second, they must be {\em learnable}: it must be feasible to find good predictions given a set of problem instances. 

To rigorously prove learnability, we follow previous work ~\cite{tim-pseudo, BalcanDDKSV19, DinitzILMV21} and focus on proving a bound on the sample complexity of finding the best predictions that generalize. 

Our main result shows that for a given problem, the pseudo-dimension of finding $k$ predictions is $\tilde{O}(k)$\footnote{$\tilde{O}(\cdot)$ suppresses logarithmic factors} factor larger than that for finding a single best predictor. We state the formal Theorem below, but defer the proof to the supplementary material. 

\begin{theorem} \label{thm:sample_complexity_multiple_predictions}
Let $\mathcal F$ be a class of functions $f: \cX \to \R$ with pseudo-dimension $d$ and let $\cF^k := \{F(x) = \min_{\ell \in [k]} f^\ell(x) \mid f^1,f^2,\ldots,f^k \in \cF\}$.  Then the pseudo-dimension of $\cF^k$ is at most $\tilde{O}(dk)$.
\end{theorem}

Note that this directly implies that the sample complexity when looking for $k$ predictions is a factor of $k$ larger than that of a single predictor by the following well-known theorem. 
\submit{
\begin{theorem} \label{thm:uniform_convergence} \cite{pollard2012convergence,anthony2009neural,tim-pseudo} 
Let $\cD$ be a distribution over a domain $X$ and $\cF$ be a class of functions $f: \cX \to [0,H]$ with pseudo-dimension $d_{\cF}$.  Consider $S$ independent samples $x_1,x_2,\ldots,x_S$ from $\cD$.  There is a universal constant $c_0$, such that for any $\epsilon > 0 $ and $\delta \in (0,1)$, if 
$S \geq c_0 \left( \frac{H}{\eps}\right)^2 (d_{\cF} + \ln(1/\delta))$
then we have 
\[
\left| \frac{1}{s} \sum_{s=1}^S f(x_i) - \E_{x \sim \cD}[f(x)] \right| \leq \epsilon
\]
for all $f \in \cF$ with probability at least $1-\delta$.
\end{theorem}
}

% TL: the line below seemed redundant
%see the supplementary material for the full proof. 
